Selective Vision is the Challenge for Visual Reasoning: A Benchmark for Visual Argument Understanding

Visual arguments, often used in advertising or social causes, rely on images to persuade viewers to do or believe something. Understanding these arguments requires selective vision: only specific visual stimuli within an image are relevant to the argument, and relevance can only be understood within the context of a broader argumentative structure. While visual arguments are readily appreciated by human audiences, we ask: are today's AI capable of similar understanding? We present VisArgs, a dataset of 1,611 images annotated with 5,112 visual premises (with regions), 5,574 commonsense premises, and reasoning trees connecting them into structured arguments. We propose three tasks for evaluating visual argument understanding: premise localization, premise identification, and conclusion deduction. Experiments show that 1) machines struggle to capture visual cues: GPT-4-O achieved 78.5% accuracy, while humans reached 98.0%. Models also performed 19.5% worse when distinguishing between irrelevant objects within the image compared to external objects. 2) Providing relevant visual premises improved model performance significantly.

==> tables/detail_caption_results.tex <==
\begin{table*}[ht]
\centering
    \centering
    \begin{tabular}{l|cc|c}
    \toprule
    & Recall & mRecall & Hit rate \\
    \midrule
    LLaVaNeXT &0.48 &0.49 &0.14 \\
    LLaVa-LLaMa3-Docci &0.27 &0.28 &0.02 \\
    ShareCaptioner &0.40 &0.41 &0.12 \\
    \toprule
    OverALL &0.38 &0.39 &0.08 \\
    \bottomrule
    \end{tabular}
    \caption{Detail Captioning models VP hit results}
    \label{tab:detail_caption_table}
\end{table*}

==> tables/safety.tex <==
\begin{table}[h]
    \centering
    \scriptsize
    \begin{tabular}{l|cc}
    \toprule
    & VP & Conclusion \\
    \midrule
    Text Safety &0.08  &0.03 \\
    Image Safety &-  &- \\
    \bottomrule
    \end{tabular}
    \caption{safety status}
    \label{tab:safety_table}
\end{table}

==> tables/task1-1_alignment.tex <==
\begin{table*}[!h]\centering
    \centering
    \scriptsize
    \begin{tabular}{l!{\color{gray!30}\vrule}rrr}
    \hline
    \multirow{1}{*}{} &\multicolumn{3}{c}{Accuracy}  \rule{0pt}{2.5ex}\\
    \hline
    &All &Cartoon &Ads \rule{0pt}{2.5ex} \\
    \hline
    \multirow{1}{*}{Clip (ViT-L/14)} &0.8285 & 0.8296 & 0.8272 \rule{0pt}{2.5ex} \\
    \hline
    \multirow{1}{*}{Clip (ViT-L/14@336px)} &0.8276 & 0.8326 & 0.8209  \rule{0pt}{2.5ex} \\
    \hline
    \multirow{1}{*}{Clip (RN50x64)} &0.8191 & 0.8272 & 0.8083
  \rule{0pt}{2.5ex}\\
    \hline
    \multirow{1}{*}{siglip(siglip-so400m-patch14-384)} &0.8643 & 0.8667 & 0.8610 \rule{0pt}{2.5ex}\\
    \hline
    \multirow{1}{*}{ofa Large} &0.7610 & 0.7918 & 0.7201  \rule{0pt}{2.5ex}\\
    \hline
    \multirow{1}{*}{ofa Base} &0.7271 & 0.7571 & 0.6875 \rule{0pt}{2.5ex}\\
    \hline
    \multirow{1}{*}{alphaclip(clip-l14-336-grit-20m)} & 0.7645 & 0.7744 & 0.7515 \rule{0pt}{2.5ex}\\
    \hline
    \end{tabular}
    \caption{VP - Bbox Alignment Accuracies}
    \label{tab:vp_alignment}
\end{table*}

==> tables/task1-2_grounding.tex <==
\begin{table*}[!h]\centering
    \centering
    \scriptsize
    \begin{tabular}{l!{\color{gray!30}\vrule}rrrr}
    \hline
    \multirow{1}{*}{} &\multicolumn{4}{c}{Accuracy}  \rule{0pt}{2.5ex}\\
    \hline
    &local iou &local score &global iou & global score \rule{0pt}{2.5ex} \\
    \hline
    \multirow{1}{*}{OFA} &0.5014 & 0.4913 & 0.4973 & 0.4882 \rule{0pt}{2.5ex} \\
    \hline
    \multirow{1}{*}{Uninext-H} &0.3875 & 0.3558 & 0.3775 & 0.3466  \rule{0pt}{2.5ex} \\
    \hline
    \multirow{1}{*}{Unified-io-2} &0.5502 & 0.5498 & 0.57779 & 0.5746
  \rule{0pt}{2.5ex}\\
    \hline
    \multirow{1}{*}{mm-g-dino} &0.4861 & 0.4715 & 0.4811 & 0.4683 \rule{0pt}{2.5ex}\\
    \hline
    \multirow{1}{*}{Lisa} & 0.4038 & 0.4061 & 0.3915 & 0.3009  \rule{0pt}{2.5ex}\\
    \hline
    \multirow{1}{*}{Groma} & & & & \rule{0pt}{2.5ex}\\
    \hline
    \end{tabular}
    \caption{VP - Bbox Grounding IOU and accuracies}
    \label{tab:vp_grounding}
\end{table*}

==> tables/task1_backup.tex <==
\begin{table*}[!h]\centering
    \centering
    \scriptsize
    \begin{tabular}{l!{\color{gray!30}\vrule}rrr}
    \hline
    \multirow{1}{*}{} &\multicolumn{3}{c}{Accuracy}  \rule{0pt}{2.5ex}\\
    \hline
    &All &Cartoon &Ads \rule{0pt}{2.5ex} \\
    \hline
    \multirow{1}{*}{Clip (ViT-L/14)} &0.8285 & 0.8296 & 0.8272 \rule{0pt}{2.5ex} \\
    \hline
    \multirow{1}{*}{Clip (ViT-L/14@336px)} &0.8276 & 0.8326 & 0.8209  \rule{0pt}{2.5ex} \\
    \hline
    \multirow{1}{*}{Clip (RN50x64)} &0.8191 & 0.8272 & 0.8083
  \rule{0pt}{2.5ex}\\
    \hline
    \multirow{1}{*}{siglip(siglip-so400m-patch14-384)} &0.8643 & 0.8667 & 0.8610 \rule{0pt}{2.5ex}\\
    \hline
    \multirow{1}{*}{ofa Large} &0.7610 & 0.7918 & 0.7201  \rule{0pt}{2.5ex}\\
    \hline
    \multirow{1}{*}{ofa Base} &0.7271 & 0.7571 & 0.6875 \rule{0pt}{2.5ex}\\
    \hline
    \multirow{1}{*}{alphaclip(clip-l14-336-grit-20m)} & 0.7645 & 0.7744 & 0.7515 \rule{0pt}{2.5ex}\\
    \hline
    \end{tabular}
    \caption{VP - Bbox Alignment Accuracies}
    \label{tab:vp_grounding}
\end{table*}

\begin{table*}[!h]\centering
    \centering
    \scriptsize
    \begin{tabular}{l!{\color{gray!30}\vrule}rrrr}
    \hline
    \multirow{1}{*}{} &\multicolumn{4}{c}{Accuracy}  \rule{0pt}{2.5ex}\\
    \hline
    &local iou &local score &global iou & global score \rule{0pt}{2.5ex} \\
    \hline
    \multirow{1}{*}{OFA} &0.5014 & 0.4913 & 0.4973 & 0.4882 \rule{0pt}{2.5ex} \\
    \hline
    \multirow{1}{*}{Uninext-H} &0.3875 & 0.3558 & 0.3775 & 0.3466  \rule{0pt}{2.5ex} \\
    \hline
    \multirow{1}{*}{Unified-io-2} &0.5502 & 0.5498 & 0.57779 & 0.5746
  \rule{0pt}{2.5ex}\\
    \hline
    \multirow{1}{*}{mm-g-dino} &0.4861 & 0.4715 & 0.4811 & 0.4683 \rule{0pt}{2.5ex}\\
    \hline
    \multirow{1}{*}{Lisa} & 0.4038 & 0.4061 & 0.3915 & 0.3009  \rule{0pt}{2.5ex}\\
    \hline
    \multirow{1}{*}{Groma} & & & & \rule{0pt}{2.5ex}\\
    \hline
    \end{tabular}
    \caption{VP - Bbox Grounding IOU and accuracies}
    \label{tab:vp_iou_grounding}
\end{table*}

==> tables/task2-2_crop.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{l|ccccc}
    \toprule
    & \multicolumn{3}{c}{Semantic} \\
    \midrule
    & All & Cartoon & Ads \\
    \midrule
    LLaVa & 76.67 & 81.17 & 72.17  \\
    LLaVa-NeXT & 82.19 & 85.57  & 78.81 \\
    InstrucBlip & 78.13 & 81.51  & 74.76 \\
    Unified-io-2 & 84.39 & 85.85  & 82.93 \\
    \hline
    \end{tabular}
    \captionof{table}{Full results of identification of premises with cropped region in semantic condition.}
\end{table*}

==> tables/task3_gpt_results_table.tex <==
\begin{table*}[!htp]
\centering
\scriptsize
\begin{tabular}{l!{\color{gray!30}\vrule}llll!{\color{gray!30}\vrule}lll!{\color{gray!30}\vrule}ll}
\hline
\multirow{2}{*}{} &\multicolumn{4}{c}{Inputs} &\multicolumn{3}{c}{Automatic} &Semantic \\
\hline
&I &VP &CP &RS &BLEU:4 &ROUGE &CIDEr &BERT \\
\hline
\multirow{3}{*}{GPT-4o} &\ding{51} & & & &3.11 &19.87 &23.11 &24.50 \\
&\ding{51} &\ding{51} & & &5.86 ($\uparrow$  2.75) &25.74 ($\uparrow$ 5.87) &43.71 ($\uparrow$ 20.61) &31.89 ($\uparrow$ 7.39) \\
&\ding{51} &\ding{51} &\ding{51} &\ding{51} &7.63 ($\uparrow$  1.77) &28.51 ($\uparrow$ 2.77) &62.03 ($\uparrow$ 18.32) &38.42 ($\uparrow$ 6.53) \\
\hline
\end{tabular}
\caption{Deduction of Conclusion Results for GPT-4o}
\label{tab:conclusion_deduction_gpt40}
\end{table*}

==> tables/task3_ic_deduction_table.tex <==
\begin{table*}[!htp]
\centering
\scriptsize
\begin{tabular}{l!{\color{gray!30}\vrule}llll!{\color{gray!30}\vrule}lll!{\color{gray!30}\vrule}ll}
\hline
\multirow{2}{*}{} &\multicolumn{4}{c}{Inputs} &\multicolumn{3}{c}{Automatic} &Semantic \\
\hline
&I &CP(P) &VP(P) &VP(N) &BLEU:4 &ROUGE &CIDEr &BERT \\
\hline
\multirow{2}{*}{LLaVA} &\ding{51} &\ding{51} &\ding{51} &\ding{51} &4.75 &25.93 &26.14 &33.88 \\
&\ding{51} &\ding{51} &\ding{51} & &6.27 &28.74 &32.82 &56.95 \\
\multirow{2}{*}{LLaVA-NeXT} &\ding{51} &\ding{51} &\ding{51} &\ding{51} &3.88 &23.83 &25.56 &25.83 \\
&\ding{51} &\ding{51} &\ding{51} & &5.62 &27.24 &31.81 &45.96 \\
\multirow{2}{*}{OFA\textsubscript{Large}} &\ding{51} &\ding{51} &\ding{51} &\ding{51} &2.89 &13.42 &14.46 &-24.02 \\
&\ding{51} &\ding{51} &\ding{51} & &4.24 &15.12 &18.30 &-38.22 \\
\multirow{2}{*}{Idefics2} &\ding{51} &\ding{51} &\ding{51} &\ding{51} &0.03 &6.17 &-16.96 &0.89 \\
&\ding{51} &\ding{51} &\ding{51} & &0.17 &6.31 &-16.74 &1.36 \\
\multirow{2}{*}{InstructBLIP} &\ding{51} &\ding{51} &\ding{51} &\ding{51} &4.14 &22.02 &20.73 &-27.28 \\
&\ding{51} &\ding{51} &\ding{51} & &5.78 &24.28 &30.08 &52.53 \\
\multirow{2}{*}{QwenVLChat} &\ding{51} &\ding{51} &\ding{51} &\ding{51} &3.94 &22.78 &23.82 &30.71 \\
&\ding{51} &\ding{51} &\ding{51} & &4.69 &24.06 &26.58 &38.88 \\
\multirow{2}{*}{CogVLM} &\ding{51} &\ding{51} &\ding{51} &\ding{51} &2.76 &20.98 &23.03 &16.13 \\
&\ding{51} &\ding{51} &\ding{51} & &3.26 &22.41 &25.59 &20.86 \\
\multirow{2}{*}{Otter} &\ding{51} &\ding{51} &\ding{51} &\ding{51} &0.93 &14.55 &11.09 &6.20 \\
&\ding{51} &\ding{51} &\ding{51} & &1.06 &15.42 &14.58 &9.70 \\
\multirow{2}{*}{Unified-io2} &\ding{51} &\ding{51} &\ding{51} &\ding{51} &5.25 &21.57 &23.67 &53.40 \\
&\ding{51} &\ding{51} &\ding{51} & &6.63 &24.10 &28.42 &67.11 \\
\end{tabular}
\caption{Deduction of Intermediate Conclusion Results for Base Models}
\label{tab:total_intermediate_conclusion_deduction}
\end{table*}

==> tables/task3_main.tex <==
\begin{table*}[!htp]
    \centering
    \small
    \begin{tabular}{ll!{\color{gray!30}\vrule}cccc!{\color{gray!30}\vrule}lll!{\color{gray!30}\vrule}ll}
    \toprule
    \multirow{3}{*}{} &&\multicolumn{4}{c}{Inputs} &\multicolumn{3}{c}{Automatic} & \multicolumn{1}{c}{Semantic} \\
    \midrule
    &&I &VP &CP &T & \multicolumn{1}{c}{Bleu-4} & \multicolumn{1}{c}{ROUGE} & \multicolumn{1}{c}{CIDEr} & \multicolumn{1}{c}{BERTScore} \\
    \midrule
    \parbox[t]{4mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{LM}}}
    %&\multirow{3}{*}{LLaMa2} & &\ding{51} & & &3.59 &23.01 &21.31 &37.11 \\
    %&& &\ding{51} &\ding{51} & &4.50 ($\uparrow$ 0.91) &25.61 ($\uparrow$ 2.60) &33.48 ($\uparrow$ 12.17) &40.90 ($\uparrow$ 3.80) \\
    %&& &\ding{51} &\ding{51} &\ding{51} &5.39 ($\uparrow$ 0.89) &27.12 ($\uparrow$ 1.50) &40.28 ($\uparrow$ 6.81) &43.98 ($\uparrow$ 3.08) \\
    &\multirow{3}{*}{LLaMa3} & &\ding{51} & & &6.40 &28.09 &37.93 &29.61 \\
    && &\ding{51} &\ding{51} & &7.78 ($\uparrow$ 1.39) &30.80 ($\uparrow$ 2.71) &54.57 ($\uparrow$ 16.65) &36.77 ($\uparrow$ 7.16) \\
    && &\ding{51} &\ding{51} &\ding{51} &8.54 ($\uparrow$ 0.76) &31.61 ($\uparrow$ 0.82) &58.88 ($\uparrow$ 4.31) &39.78 ($\uparrow$ 3.01) \\
    &\multirow{3}{*}{Mistralv0.2} & &\ding{51} & & &2.48 &18.30 &18.41 &19.31 \\
    && &\ding{51} &\ding{51} & &4.54 ($\uparrow$ 2.06) &23.88 ($\uparrow$ 5.57) &34.83 ($\uparrow$ 16.42) &29.57 ($\uparrow$ 10.25) \\
    && &\ding{51} &\ding{51} &\ding{51} &6.28 ($\uparrow$ 1.74) &27.39 ($\uparrow$ 3.51) &47.58 ($\uparrow$ 12.75) &35.89 ($\uparrow$ 6.33) \\
    &\multirow{3}{*}{Zephyr} & &\ding{51} & & &2.31 &15.28 &19.10 &19.41 \\
    && &\ding{51} &\ding{51} & &3.26 ($\uparrow$ 0.95) &17.47 ($\uparrow$ 2.18) &28.59 ($\uparrow$ 9.49) &26.13 ($\uparrow$ 6.72) \\
    && &\ding{51} &\ding{51} &\ding{51} &5.94 ($\uparrow$ 2.67) &24.65 ($\uparrow$ 7.18) &45.84 ($\uparrow$ 17.25) &34.05 ($\uparrow$ 7.92) \\
    \midrule
    \parbox[t]{4mm}{\multirow{36}{*}{\rotatebox[origin=c]{90}{MLM}}}
    &\multirow{4}{*}{OFA} &\ding{51} & & & &0.00 &0.27 &0.01 &-21.08 \\
    &&\ding{51} &\ding{51} & & &0.00 (-) &5.26 ($\uparrow$ 4.99) &0.39 ($\uparrow$ 0.38) &-15.39 ($\uparrow$ 5.68) \\
    &&\ding{51} &\ding{51} &\ding{51} & &0.00 (-) &6.81 ($\uparrow$ 1.55) &0.32 ($\downarrow$ 0.06) &-13.66 ($\uparrow$ 1.73) \\
    &&\ding{51} &\ding{51} &\ding{51} &\ding{51} &0.00 (-) &7.36 ($\uparrow$ 0.55) &0.65 ($\uparrow$ 0.32) &-12.44 ($\uparrow$ 1.22) \\
    & \multirow{4}{*}{LLaVA} &\ding{51} & & & &1.50 &16.01 &3.65 &6.50 \\
    &&\ding{51} &\ding{51} & & &3.86 ($\uparrow$ 2.36) &22.88 ($\uparrow$ 6.87) &18.69 ($\uparrow$ 15.04) &20.60 ($\uparrow$ 14.10) \\
    &&\ding{51} &\ding{51} &\ding{51} & &5.54 ($\uparrow$ 1.69) &26.93 ($\uparrow$ 4.05) &34.84 ($\uparrow$ 16.14) &29.53 ($\uparrow$ 8.94) \\
    &&\ding{51} &\ding{51} &\ding{51} &\ding{51} &6.63 ($\uparrow$ 1.09) &28.19 ($\uparrow$ 1.26) &44.64 ($\uparrow$ 9.80) &33.28 ($\uparrow$ 3.75) \\
    &\multirow{4}{*}{LLaVA-NeXT} &\ding{51} & & & &3.23 &21.62 &13.51 &15.34 \\
    &&\ding{51} &\ding{51} & & &6.35 ($\uparrow$ 3.12) &28.09 ($\uparrow$ 6.47) &36.09 ($\uparrow$ 22.58) &28.16 ($\uparrow$ 12.83) \\
    &&\ding{51} &\ding{51} &\ding{51} & &7.42 ($\uparrow$ 1.07) &30.21 ($\uparrow$ 2.12) &47.64 ($\uparrow$ 11.55) &33.93 ($\uparrow$ 5.76) \\
    &&\ding{51} &\ding{51} &\ding{51} &\ding{51} &8.46 ($\uparrow$ 1.04) &31.69 ($\uparrow$ 1.49) &61.14 ($\uparrow$ 13.50) &38.61 ($\uparrow$ 4.68) \\
    
    &\multirow{4}{*}{Idefics2} &\ding{51} & & & &3.50 &21.74 &16.07 &15.75 \\
    &&\ding{51} &\ding{51} & & &4.13 ($\uparrow$ 0.64) &23.84 ($\uparrow$ 2.11) &25.00 ($\uparrow$ 8.92) &21.98 ($\uparrow$ 28.65) \\
    &&\ding{51} &\ding{51} &\ding{51} & &5.50 ($\uparrow$ 1.37) &25.78 ($\uparrow$ 1.93) &34.64 ($\uparrow$ 9.64) &28.33 ($\uparrow$ 9.96) \\
    &&\ding{51} &\ding{51} &\ding{51} &\ding{51} &7.82 ($\uparrow$ 2.32) &29.15 ($\uparrow$ 3.37) &53.84 ($\uparrow$ 19.20) &35.39 ($\uparrow$ 0.28) \\
    &\multirow{4}{*}{InstructBLIP} &\ding{51} & & & &0.00 &3.80 &0.75 &-10.85 \\
    &&\ding{51} &\ding{51} & & &2.53 ($\uparrow$ 2.53) &18.94 ($\uparrow$ 15.14) &16.35 ($\uparrow$ 15.60) &17.80 ($\uparrow$ 33.01) \\
    &&\ding{51} &\ding{51} &\ding{51} & &5.33 ($\uparrow$ 2.80) &26.91 ($\uparrow$ 7.98) &36.87 ($\uparrow$ 20.52) &27.77 ($\uparrow$ 9.80) \\
    &&\ding{51} &\ding{51} &\ding{51} &\ding{51} &6.18 ($\uparrow$ 0.85) &28.29 ($\uparrow$ 1.38) &42.53 ($\uparrow$ 5.65) &28.04 ($\uparrow$ 1.04) \\
    &\multirow{4}{*}{QwenVLChat} &\ding{51} & & & &0.62 &13.50 &6.60 &12.94 \\
    &&\ding{51} &\ding{51} & & &3.66 ($\uparrow$ 3.04) &24.33 ($\uparrow$ 10.83) &25.15 ($\uparrow$ 18.54) &22.96 ($\uparrow$ 10.01) \\
    &&\ding{51} &\ding{51} &\ding{51} & &4.58 ($\uparrow$ 0.92) &26.55 ($\uparrow$ 2.23) &31.61 ($\uparrow$ 6.46) &29.33 ($\uparrow$ 6.37) \\
    &&\ding{51} &\ding{51} &\ding{51} &\ding{51} &4.85 ($\uparrow$ 0.26) &27.31 ($\uparrow$ 0.76) &35.62 ($\uparrow$ 4.01) &31.41 ($\uparrow$ 2.08) \\
    &\multirow{4}{*}{CogVLM} &\ding{51} & & & &4.93 &25.73 &25.13 &25.53 \\
    &&\ding{51} &\ding{51} & & &5.81 ($\uparrow$ 0.88) &27.86 ($\uparrow$ 2.13) &36.13 ($\uparrow$ 11.00) &29.95 ($\uparrow$ 4.42) \\
    &&\ding{51} &\ding{51} &\ding{51} & &6.86 ($\uparrow$ 1.04) &29.42 ($\uparrow$ 1.56) &43.23 ($\uparrow$ 7.10) &32.91 ($\uparrow$ 2.96) \\
    &&\ding{51} &\ding{51} &\ding{51} &\ding{51} &7.77 ($\uparrow$ 0.92) &30.76 ($\uparrow$ 1.34) &52.14 ($\uparrow$ 8.90) &35.07 ($\uparrow$ 2.16) \\

    &\multirow{4}{*}{Unified-io 2} &\ding{51} & & & &0.04 &9.61 &0.68 &-9.87 \\
    &&\ding{51} &\ding{51} & & &0.61 ($\uparrow$ 0.57) &13.30 ($\uparrow$ 3.69) &4.07 ($\uparrow$ 3.39) &-3.40 ($\uparrow$ 6.47) \\
    &&\ding{51} &\ding{51} &\ding{51} & &0.74 ($\uparrow$ 0.12) &14.63 ($\uparrow$ 1.33) &6.72 ($\uparrow$ 2.66) &4.23 ($\uparrow$ 7.63) \\
    &&\ding{51} &\ding{51} &\ding{51} &\ding{51} &1.10 ($\uparrow$ 0.37) &16.27 ($\uparrow$ 1.64) &11.21 ($\uparrow$ 4.48) &8.01 ($\uparrow$ 3.78) \\
    %&\multirow{4}{*}{Otter} &\ding{51} & & & &2.34 &19.58 &4.71 &25.96 \\
    %&&\ding{51} &\ding{51} & & &3.75 ($\uparrow$ 1.41) &24.89 ($\uparrow$ 5.31) &19.29 ($\uparrow$ 14.59) &38.07 ($\uparrow$ 12.11) \\
    %&&\ding{51} &\ding{51} &\ding{51} & &3.82 ($\uparrow$ 0.07) &24.98 ($\uparrow$ 0.09) &18.09 ($\downarrow$ 1.21) &39.02 ($\uparrow$ 0.95) \\
    %&&\ding{51} &\ding{51} &\ding{51} &\ding{51} &4.06 ($\uparrow$ 0.24) &24.69 ($\downarrow$ 0.28) &17.81 ($\downarrow$ 0.28) &37.96 ($\downarrow$ 1.05) \\
    &\multirow{3}{*}{GPT-4-O} &\ding{51} & & & & 3.11 & 19.87 & 23.11 & 24.50 \\ 
    &&\ding{51} &\ding{51} & & &5.86 ($\uparrow$ 2.75) & 25.74 ($\uparrow$ 5.87) & 43.71 ($\uparrow$ 20.61) & 31.89 ($\uparrow$ 7.39) \\
    &&\ding{51} &\ding{51} &\ding{51} &\ding{51} & 7.63 ($\uparrow$ 1.77) & 28.51 ($\uparrow$ 2.77) & 62.03 ($\uparrow$ 18.32) & 38.42 ($\uparrow$ 6.53) \\
    \bottomrule
    \end{tabular}
    \caption{Deduction of Conclusion Results for Base Models}
    \label{tab:task3}
\end{table*}
